A GPU-accelerated Molecular Docking Workflow with Kubernetes and Apache Airflow

Complex workflows play a critical role in accelerating scientific discovery. In many scientific domains, efficient workflow management can lead to faster scientific output and broader user groups. Workflows that can leverage resources across the boundary between cloud and HPC are a strong driver for the convergence of HPC and cloud. This study investigates the transition and deployment of a GPU-accelerated molecular docking workflow that was designed for HPC systems onto a cloud-native environment with Kubernetes and Apache Airflow. The case study focuses on state-of-of-the-art molecular docking software for drug discovery. We provide a DAG-based implementation in Apache Airflow and technical details for GPU-accelerated deployment. We evaluated the workflow using the SWEETLEAD bioinformatics dataset and executed it in a Cloud environment with heterogeneous computing resources. Our workflow can effectively overlap different stages when mapped onto different computing resources.

==> backup.tex <==
\subsection{iPIC3D}

In this workflow, a plasma simulation performs classical particle-in-cell methods to update particle position and velocity by first principle. A supervised machine-learning model is employed to perform classification of electron trajectories to identify regions of interest and different acceleration 

One of the most powerful and successful tools for performing plasma simulations is the PIC method. In summary, the PIC method determines the trajectories of particles (electrons and protons) under the effect of a self-consistent electromagnetic field: electrons and protons generate electric and magnetic fields that act on particles themselves. 

In this work, we use sputniPIC~\cite{chien2020sputnipic}, the successor of the iPIC3D code \cite{markidis2010multi,peng2015energetic}, to generate the particle trajectory dataset. The sputniPIC code is based on the implicit discretization of governing equations for electromagnetic kinetic equations of particles: particle equation of motion and Maxwell equations. The main computational kernel is the so-called \emph{particle mover} or \emph{pusher} that updates particle position and velocity by solving the equation of motion. Instead of the more common leap-frog or Boris particle mover~\cite{birdsall2004plasma}, we use a predictor-corrector scheme to solve the average particle velocity $\mathbf{\bar{v}}_p = (\mathbf{v}_p^{n} + \mathbf{v}_p^{n+1})/2$ during the time step $\Delta t$ with $n$ indicating the time level:
\begin{eqnarray}
\label{vhat2}
\tilde{\mathbf{v}}_p&=&\mathbf{v}_p^n+\frac{q\Delta t}{2m}\mathbf{\bar{E}}_p\\
\label{vn+1/2}
\mathbf{\bar{v}}_p&=&\frac{\tilde{\mathbf{v}}_p+\frac{q\Delta
t}{2m c}\bigl(\tilde{\mathbf{v}}_p\times\mathbf{\bar{B}}_p+\frac{q\Delta
t}{2m c}(\tilde{\mathbf{v}}_p\cdot\mathbf{\bar{B}}_p)\mathbf{\bar{B}}_p\bigr)}{(1+\frac{q^2\Delta t^2}{4m^2c^2}{\bar{B}_p}^2)},
\end{eqnarray}

where $p$ is the particle index, $q,m$ are the particle charge and mass, and $c$ is the speed of light in vacuum.
The number of iterations to determine $\mathbf{\bar{v}}_p$ is either set by a prescribed error tolerance or fixed to a small number of iterations. In this work, we use three iterations for both electron and proton particles.  The $\mathbf{\bar{v}}_p$ calculation requires the electric and magnetic field at the particle position, $\mathbf{E}_p$ and $\mathbf{B}_p$. However, the electric and magnetic field values, $\mathbf{E}_g$ and $\mathbf{B}_g$ are only defined at the grid points in the PIC method. To calculate these quantities, the PIC method uses the linear weight or interpolation functions $W({\bf x}_g-{\bf x}_p)$ defined as follows:
\begin{equation}
\label{interpW}
W({\bf x}_g-{\bf x}_p) =
\left\{
\begin{array}{l}
 1 - |{\bf x}_g-{\bf x}_p|/\Delta x \quad \textup{if} \quad |{\bf x}_g-{\bf x}_p| < \Delta x \\
0  \quad \textup{otherwise}  .\end{array}
\right.
\end{equation}
With the usage of interpolation functions, we can calculate the electric and magnetic field at the particle position from these values on the grid point $g$:
\begin{equation}
{\bf E}_p=\sum_g^{N_g} {\bf E}_g W({\bf x}_g-{\bf x}_p) \quad \quad {\bf B}_p=\sum_g^{N_g} {\bf B}_g W({\bf x}_g-{\bf x}_p) .
\label{interp}
\end{equation}
Once the particle average velocity is calculated, each particle position and velocity is updated as follows:
\begin{equation}
\label{dif_eom2}
\left\{
\begin{array}{l}
\mathbf{v}_p^{n+1} = 2 \mathbf{\bar{v}}_p - \mathbf{v}_p^{n}  \\
\mathbf{x}_p^{n+1} = \mathbf{x}_p^{n} + \mathbf{\bar{v}}_p\Delta t.
\end{array} 
\right. 
\end{equation}
Detailed descriptions of mathematical derivation of the implicit discretized equations can be found in~\cite{markidis2014fluid,markidis2011energy}. The typical PIC simulations run on supercomputers, possibly with accelerators, and uses millions of particles.

==> related-backup.tex <==
\section{Related Works}
%\todo{Jacob and Gabin}

\paragraph{Scientific workflow platforms.} Aside the HPC workflows platforms discussed in Section \ref{sec:hpcwf}, there are other specialized frameworks that provides additional features and usability for scientific workflows on HPC systems. Some of the relevant works in this field are Pegasus~\cite{Deelman2005,Deelman2016}, Taverna~\cite{Wolstencroft2013}, FireWorks~\cite{Jain2015}, RADICAL-Pilot~\cite{Merzky2015}, Nextflow~\cite{DiTommaso2017}, signac~\cite{Adorf2018}, and CRCPs~\cite{Rosa2021}. Additionally, Pegasus and Nextflow can also be deployed in cloud environments; the former can be deployed on cloud as an HTCondor instance while the latter has support to other platforms such as Kubernetes, Azure Cloud and Google Cloud. Computational Resource and Cost Prediction service~\cite{Rosa2021} allows users to control the financial costs of workflow execution on federated clouds. %\todo{Focus this on which have cloud support}

\paragraph{Application workflows.} Complex workflows appear in many scientific domains. In climate modeling, multiple models such as atmosphere, ice, and river are coupled into one workflow~\cite{Chen2017}. In medicine, molecular docking workflows are used for drug discovery~\cite{Glaser2021,Darme2021,Saadi2021,Gadioli2022,Venkatraman2022}. In materials science, classical density functional theory has been combined with machine learning and Monte Carlo simulation to understand the thermodynamics of novel alloys~\cite{Liu2021}. In structural biology, multiple scales of simulations and machine learning methods have furthered understanding of the structure of viruses~\cite{Trifan2022}, and protein folding~\cite{Gao2022}. In geoscience, workflows for earthquake and tsunami simulations have been composed for geohazard risk prediction~\cite{Cordrie2023}. In fusion physics, simulation, analysis and visualize have been combined to enable online visualization of simulation data~\cite{Suchyta2022}.



\paragraph{HPC workloads in cloud environments.} Several works have explored how HPC workloads can be executed in cloud environments. Saha, et al.~\cite{saha2018evaluation} evaluated the Singularity containerization platform and Docker Swarm was used as an orchestrator, focusing on network mapping for MPI. %  The results displays that the overall performance is not much impacted due to the usage of containers.%, except in some specific conditions (e.g., running a rank per container will have a degradation performance of over 50\%).
Beltre, et al.~\cite{beltre2019enabling} run MPI workloads over TCP/IP and InfiniBand (RDMA) communication and measure the overheads between different container orchestrators. They compare Kubernetes, Docker Swarm and baremetal. They find that overhead for Docker Swarm is comparable to baremetal and Kubernete's overhead, for applications that communicates TCP/IP, can be up to 13\%. 
Misale, et al.~\cite{misale2021towards} proposes a scheduler for Kubernetes (“KubeFlux”) based on the ideas from the Flux scheduler. Kubernetes can run multiple schedulers and will go to KubeFlux when explicitly specified. The used infrastructure for testing was Amazon's with three control planes and seven worker nodes. Two results are presented: KubeFlux over Flux and KubeFlux over Kubernetes. For the former, it schedules 471 pods and takes about 10\% of the Flux execution time. For the latter case, it relies on metrics from the pod lifecycle that has a granularity of seconds.

%\textbf{Performance measurements and analysis.} Sukhija, et al.~\cite{sukhija2019towards}  proposes the integration of a tool called OMNI (from NERSC) with current state-of-art tools that are used in cloud computing settings, such as Prometheus (for data scrapping) and Grafana (visualization). The major contribution of the paper is the discussions of the requirements of a monitoring tool into HPC environment. Zhou, et al.~\cite{zhou2021container}


==> setup.tex <==
\section{Experiment Environment}
\label{experiments}

\textbf{Hardware Infrastructure.} The cloud testbed has an Intel i7-7820X processor at 3.6 GHz, with 16 cores in total, and 32 GB of DD4 memory at 2133 MHz. In terms of storage, the system contains an Intel Optane SSD 900p with 480 GB, a Kingston UV400 SSD, 2x Seagate Barracuda with 2 TB each and a Samsung EVO NVMe driver with 1 TB. The server also includes an Intel I219-V single-port 1 gigabyte Ethernet controller, and NVIDIA RTX 2060 Super GPUs. The GPU follows the "Turing" architecture containing tensor cores and GDDR6 memory, having a theoretical peak performance of 201 GFlops/s for double precision operations.  

\textbf{Software Infrastructure.} The server runs Ubuntu 22.04 operating system with the default Linux kernel 5.19. The testbed runs k3d to emulate a Kubernetes v1.23 cluster. In order to allow k3d to access the GPU resources, a custom image with support to Nvidia's CUDA (\texttt{libnvidia-container-tools} and \texttt{libnvidia-container-runtime}) was built and used upon cluster creation. Docker was also setup to use the Nvidia runtime by default. 

The Airflow used in the experiments was deployed using the set of helm charts officially supported by the community. Airflow version is 1.8.0 and the backend uses PostgreSQL 12.1 for storing the relevant data. The deployment of containers was done in Python using Airflow's \texttt{KubernetesPodOperator} interface together with Kubernetes' own API.

==> workflow-pic.tex <==
\section{In-situ Plasma Simulation and Classification Workflow}
The particle-in-cell method is a technique devised during the late 50s to solve certain classes of partial differential equations. 

There are many open source implementation variants of the PIC method, e.g. iPiC3D~\cite{MARKIDIS20101509}, VPIC~\cite{bowers2008ultrahigh}, Warp-X~\cite{VAY2018476} and PiConGPU~\cite{10.1145/2503210.2504564}.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.45]{figures/autodock_dag_wf1_alt.png}
    \caption{DAG model of the four tasks in iPIC3D and a data analysis task.}
    \label{fig:autodock}
\end{figure}

\subsection{PIC Workflow on Airflow} % This is pretty much repeating from the AutoDock part
Similarly to Section \ref{sec:autodockaf}, there was also the need to build a specific Docker image with all the dependencies of sputniPIC in order to deploy the application. The pod description in the DAG was done similarly as AutoDock-GPU, with the exclusion of GPU-related information. After this, the application was ready to be integrated into our workflow.

\subsection{Preliminary Results}
